In the Search of Optimal Concurrency

Implementing a concurrent data structure typically begins with defining its sequential specification. However, when used \emph{as is}, a nontrivial sequential data structure, such as a linked list, a search tree, or a hash table, may expose incorrect behavior: lost updates, inconsistent responses, etc. To ensure correctness, portions of the sequential code operating on the shared data must be "protected" from data races using synchronization primitives and, thus, certain schedules of the steps of concurrent operations must be rejected. But can we ensure that we do not "overuse" synchronization, i.e., that we reject a concurrent schedule only if it violates correctness? In this paper, we treat this question formally by introducing the notion of a \emph{concurrency-optimal} implementation. A program's concurrency is defined here as its ability to accept concurrent schedules, i.e., interleavings of steps of its sequential implementation. An implementation is concurrency-optimal if it accepts all interleavings that do not violate the program's correctness. We explore the concurrency properties of \emph{search} data structures which can be represented in the form of directed acyclic graphs exporting insert, delete and search operations. We prove, for the first time, that \emph{pessimistic} e.g., based on conservative locking) and \emph{optimistic serializable} e.g., based on serializable transactional memory) implementations of search data-structures are incomparable in terms of concurrency. Specifically, there exist simple interleavings of sequential code that cannot be accepted by \emph{any} pessimistic (and \emph{resp.}, serializable optimistic) implementation, but accepted by a serializable optimistic one (and \emph{resp.}, pessimistic). Thus, neither of these two implementation classes is concurrency-optimal.

==> lin-locproof.tex <==
In this section, we introduce the locally-serializable
linearizability correctness criterion, or \LS-linearizability. 
Informally, a schedule is \LS-linearizable if 
the history of invocations and responses
constitute a sequential total order, while every local schedules is
consistent with some sequential schedule.
Then we show that \LS-linearizability is \emph{local} (i.e., holds
under composition) and \emph{non-blocking} (i.e., can be implemented
without locks)~\cite{HW90}.

A \emph{complete schedule} is a schedule in which every invocation of
a high-level operation, every \emph{read} and every \emph{write} has a matching response.
%
A \emph{completion of ${SC}$} is a complete extension of
${SC}$ that is constructed by adding to $SC$ events of 
pending operations (read, writes and high-level responses).  
%Informally, we complete schedule by allowing each pending operation of  
%to perform steps (as in a sequential implementation) until it terminates.
%% We assume that a schedule can be completed only by completing
%%pending operations i.e. no new invocation events can be added to the completion.
%%Note that a finite schedule has infinitely many completions.
%%
\begin{definition}
\label{def:lin}
Let ${I}_{S}$ be a sequential implementation of an object of type
$\tau$ and $\Sigma$ be the set of \emph{sequential schedules} of $I_S$.
A complete schedule ${SC}$ is \emph{\LS-linearizable with respect to ${I}_{S}$} if 
\begin{itemize}
\item the history $H$ of $SC$ 
%that consists of only the invocations and responses of high-level operations 
is \emph{linearizable with respect to $\tau$} 
\item for each $p_i$, 
$i \in \{1,\ldots , n\}$, there exists $S_i \in \Sigma$ such that $SC|p_i=S_i|p_i$.
%\footnote{Note that, since we assume that no complete operation is empty, the last item implies that $SS$, the sequential
%\emph{linearization} of $SC$, also preserves the real-time order of
%high-level operations in $SC$.}   
\end{itemize}
\end{definition}
%We say that a schedule ${SC}$ of an implementation of an object $O$ of type $\tau$ \emph{allows} a history $H$ of $O$ if ${SC}$ reduced to the invocation and response events of the operations of $O$ is equivalent to $H$. 
%The first condition is the same as Definition~\ref{def:linh} while
%the second condition requires that the local schedule of each process
%looks  consistent with some sequential schedule of $I_S$.
%% 
We say that an object implementation ${I}$ is \LS-linearizable with respect to ${I}_{S}$
if every schedule exported by $I$ has a
\LS-linearizable (with respect to $I_S$) completion.
%to obtain a linearization with respect to the given sequential
%implementation ${I}_{S}$ of the object, 
%
%

Note that since an \LS-linearizable implementation (with respect to $I_S$) can be treated by
every user as $I_S$, no operation can do somethiong not
allowed by $I_S$  (e.g., division by zero or infinite loops).    



%\begin{definition}
%\label{def:block}
A correctness property $\mathcal{P}$ on schedules is \emph{non-blocking}~\cite{HW90}
if a schedule $SC$ satisfies $\P$ and contains a pending invocation
$i_{op}$ of a high-level operation $op$,  there exists a schedule $\sigma$ containing only
events of $op$ and ending with a matching response $r_{op}$ such that 
$SC\cdot r\sigma$ satisfies $\mathcal{P}$.
%\end{definition}
%
\begin{theorem}
\label{th:block}
\LS-linearizability is non-blocking.
\end{theorem}
%
%
\begin{proof}
%
Let $I_S$ be a sequential implementation of an object of type
$\tau$. 
%Recall that we assume $\tau$ to be \emph{total}.
%, so every pending invocation $i_{op}$ of a high-level operation $op$ has a matching response $r_{op}$.

Let ${\bar{SC}}=SC\cdot SC'$ denote an \LS-linearizable (w.r.t. $I_S$) completion of a
partial history $SC$, $L$ be the sequential history that linearizes
$SC$ and, for each $p_i$, $S_i$ be the sequential schedules of $I_S$ such that
$S_I|p_i=\bar{SC}|p_i$. 
Let $SC$ contain a pending invocation  $op$ of a high-level operation $OP$. 
We construct $SC''$ by permuting events in $SC'$ so that 
$\bar{SC}'$ begins with all events of $op$ that are present in
$SC'$ (ending with a matching response $r_{op}$) such that 
${SC}''|p_i={SC}'|p_i$, for each $p_i$.
(Essentially, we simply shift all events on behalf of $op$ to the
beginning of $SC'$.)    

We claim that the resulting schedule $SC\cdot SC''$ is
\LS-linearizable. 
Since $\bar{SC}$  and $SC\cdot SC''$ agree on the local histories, 
we have $S_i|p_i=SC\cdot SC"|p_i$.
Moreover, since we obtained $SC\cdot SC''$ by only reordering events of operations that were
concurrent in $\bar{SC}$, we obtain that  $op'\rightarrow_{\bar{SC}} op''$ if and only if  $op'\rightarrow_{SC\cdot SC''} op''$.
Thus, $L$ is a valid linearization of $SC\cdot SC"$.
 
But $SC\cdot SC''$ is a completion of $SC\cdot\sigma$, where $\sigma$
only contains events of $op$ and ends with a matching response $r_{op}$.
Thus, $SC\cdot\sigma$ is \LS-linearizable (w.r.t. $I_S$).
\end{proof}
%

The \emph{locality} feature of a correctness property~\cite{HW90} says that
if a system composed of multiple object implementations is correct,
with respect to every object, then it is correct with respect to the
object composition.   
Formally, every sequential implementation $I_S$ of an object  $O_1\times O_2$ of a
composed type $\tau_1\times\tau_2$ naturally induces two sequential
implementations $I_{S1}$ and $I_{S2}$ of objects $O_1$ and $O_2$,
respectively. 
Now a correctness property $\mathcal{P}$ is \emph{local} if for every
schedule $SC$ on an object composition $O_1\times O_2$ 
if $\P$ holds for $SC|O_i$ with
respect to $I_{Si}$, for $i=1,2$, then $\P$ holds for $SC$ with
respect to $I_S=I_{S1}\times I_{S2}$.
Here $SC|O_i$ denotes the  subsequence of $SC$ consisting of steps on $O_i$.
    
%
\begin{theorem}
\label{th:local}
\LS-linearizability is local. 
\end{theorem}
%
\begin{proof}
%
Let $SC$, a schedule on $O_1\times O_2$  be \LS-linearizable
with respect to $I_S$. 
Let each $SC|O_i$, $i=1,2$, be \LS-linearizable with respect to $I_{Si}$. 
Without loss of generality,  we assume that $SC$ is complete (if $SC$
is incomplete, we consider any completion of it containing
\LS-linearizable completions of  $SC|O_1$ and $SC|O_1$.

Let $H$ be  the history of $SC$.
Let $L_1$ and $L_2$ be linearizations of the histories of $H|O_1$
and $H|O_2$, respectively. 
Consider the relation $LI=\rightarrow_{L_1}\cup\rightarrow_{L_2}$ defined
on the operations of $SC$ (the union of real-time orders on $L_1$ and $L_2$).     
Since $\rightarrow_{L_1}$ and $\rightarrow_{L_2}$ are defined on
distinct sets of operations of $SC$, we observe that  $LI$ is a (strict)
partial order. 
%i.e., asymmetric, irreflexive and transitive. 

Let $PO$ denote the relation $LI\cup\rightarrow_{H}$.
We show $PO$ contains no cycles and, thus, since both $LI$ and $\rightarrow_H$
are irreflexive and asymmetric, can be extended to a total order.

Suppose not, i.e., there is a chain of operations $o_0,\ldots,o_k$
($k>1$) in $SC$ such that $o_0=o_k$ and $(o_i,o_{i+1})\in PO$, for
$i=1,\ldots,k-1$. 
Since  $LI$ and $\rightarrow_{H}$
are partial orders and, thus, transitive, here must be at least one link in
the chain, $(o_j,o_j+1)$ such that  $o_j\rightarrow_{H}o_{j+1}$.
Without loss of generality assume that $j=0$.
Moreover, since $L_1$ and $L_2$ are defined on distinct sets of
operations, the edges in the chain alternate between $\rightarrow_{H}$
and $\rightarrow_{L_i}$ (for $i=1,2$).

We show, by induction, that, for all $i=1,\ldots,k$, we have
$o_i\nrightarrow_Ho_1$.
Clearly, $o_2\nrightarrow_Ho_1$ ($LI$ is consistent with $\rightarrow_H$).
Let the hypothesis hold for all $2<i<k$ and suppose, by contradiction,
that $o_k\rightarrow_H o_1$. 

Consider two possible cases. If $o_{k-1}\rightarrow_H o_k$, then, by
transitivity of $\rightarrow_H$, we have $o_{k-1}\rightarrow_Ho_1$---a contradiction. 

If  $o_{k-1}\rightarrow_{L_i} o_k$ for some some $i=1,2$, 
then, since the edges of the chain alternate  between $\rightarrow_{H}$ and $\rightarrow_{L_j}$, we
have $o_{k-2}\rightarrow_Ho_{k-1}$ and, thus, 
$o_{k-2}$ ends before $o_{k_1}$ begins in $H$. 
By the inductive assumption, we have  $o_{k-2}\nrightarrow_Ho_{1}$,
and thus  $o_{1}$ begins before $o_{k-2}$ ends in $H$.
Since $\rightarrow_{L_i}$ is consistent with $\rightarrow_H$,   
$o_{k}\nrightarrow_Ho_{k-1}$ and, thus, $o_{k-1}$
begins before $o_k$ ends in $H$. 
Finally, we obtain  that $o_1$ begins before $o_k$ ends and, thus, 
 $o_{k}\nrightarrow_Ho_{1}$. 
But $o_k=o_0 \rightarrow_Ho_{1}$---a contradiction.

Hence, $PO$ can be extended to a total order, which implies a
linearization of $H$.

Now let, for each process $p_i$, $S_i^1$ and $S_i^2$ be two sequential schedules of
$I_{S1}$ and $I_{S2}$  such that $SC|p_i|O_j=S_i^j|p_i$, for $j=1,2$
(since $SC|O_2$ and $SC|O_2$ are \LS-linearizable such schedules exist).
We construct a sequential schedule $S_i$ by interleaving events of
$S_i^1$ and $S_i^2$ so that $S_i|O_j=S_i^j$, $j=1,2$. 
Since each $S_i^j$ acts on a distinct component $O_j$ of $O_1\times
O_2$, every such $S_i$ is a sequential schedule of $I_S$.
We pick one $S_i$ that respect the local schedule $SC|p_i$,
which is possible, since $SC|p_i$ is consistent with both    
$S_1|p_i$ and $S_2|p_i$. 

Thus, for each $p_i$, we obtain a schedule of $I_S$ that agrees with
$SC|p_i$. Thus, $SC$ is \LS-linearizable. 
\end{proof}
%


==> prel.tex <==
%!TEX root = 0main.tex
\section{Preliminaries}
\label{sec:prel}
%
\vspace{1mm}\noindent\textbf{Sequential types and implementations.}
%
An \emph{object type} $\tau$ is a tuple
$(\Phi,\Gamma, Q, q_0, \delta)$ where
$\Phi$ is a set of operations,
$\Gamma$ is a set of responses, $Q$ is a set of states, $q_0\in Q$ is an
initial state and 
$\delta \subseteq Q\times \Phi \times Q\times \Gamma$ 
is a transition relation that determines, for each state
and each operation, the set of possible
resulting states and produced responses~\cite{AFHHT07}. 
Here, $(q,\pi,q',r) \in \delta$ implies that when
an operation $\pi \in \Phi$ is applied on an object of type $\tau$
in state $q$, the object moves to state $q'$ and returns a response $r$.
We consider only types that are \emph{total}
 i.e., for every $q\in Q$,
$\pi \in \Phi$, there exist  $q' \in Q$ and
$r\in \Gamma$ such that $(q,\pi,q',r) \in \delta$.
We assume that every type $\tau=(\Phi,\Gamma, Q, q_0, \delta)$ is \emph{computable}, i.e., 
there exists a Turing machine that, 
for each input $(q,\pi)$, $q \in Q$, $\pi\in \Phi$, computes
a pair $(q',r)$ such that $(q,\pi,q',r) \in \delta$.

For any type $\tau$, each high-level object $O_{\tau}$ of this type has a \emph{sequential implementation}. 
For each operation $\pi \in \Phi$, 
$\id{IS}$ specifies a deterministic procedure that 
performs \emph{reads} and \emph{writes} on a collection of objects
$X_1,\ldots , X_m$ that encode a state of $O_{\tau}$, and returns a response $r\in \Gamma$. 

\vspace{1mm}\noindent\textbf{Concurrent implementations.}
We tackle the problem of turning the sequential
implementation $\id{IS}$ of type $\tau$ into a \emph{concurrent} one, shared by 
$n$ \emph{processes} $p_1,\ldots,p_n$ ($n\in\Nat$).
The implementation provides the processes with algorithms 
for the reads and writes on objects.
We refer to the resulting implementation as a concurrent implementation of $(\id{IS},\tau)$.
We assume an asynchronous shared-memory system in which the processes communicate by
applying primitives on shared \emph{base objects}~\cite{Her91}.
We place no upper bounds on the number of versions an object may maintain or on the size of base objects.
Throughout this paper, the term \emph{operation} refers to some
high-level operation of the type, 
while read-write operations on objects are referred simply 
as \emph{reads} and \emph{writes}.

An implemented read or write may \emph{abort} by returning a special response
$\bot$. In this case we say that the corresponding high-level
operation is \emph{aborted}. 
The $\bot$ event is treated both as the response event of the read or
write operation and as the response of the corresponding high-level operation.   

\vspace{1mm}\noindent\textbf{Executions and histories.}
An \emph{execution} of a concurrent implementation is a sequence
of invocations and responses of high-level operations of type $\tau$, %(atomic) 
invocations and responses of read and write
operations, and invocations and responses of base-object primitives.
%Throughout this paper,  the term \emph{operation} refers to some
%high-level operation of the type, 
%while reads and writes on objects are referred as \emph{read} (and resp. \emph{write}) operations.
%%\emph{synchronization} primitives (e.g., lock acquisitions and
%%releases or transaction delimiters). 
%%A \emph{step} in an execution corresponds to one of the above events.
We assume that executions are \emph{well-formed}:
no process invokes a new read or write, or high-level operation before
the previous read or write, or a high-level operation, resp., 
returns, or takes steps outside its read or write operation's interval.

Let $\alpha|p_i$ denote the subsequence of an execution $\alpha$
restricted to the events of process $p_i$.
Executions $\alpha$ and $\alpha'$ are \emph{equivalent} if for every process
$p_i$, $\alpha|p_i=\alpha'|p_i$.
An operation $\pi$ \emph{precedes} another operation $\pi'$ in an execution
$\alpha$, 
denoted $\pi \rightarrow_{\alpha} \pi'$, 
if the response of $\pi$ occurs before the invocation of $\pi'$.
Two operations are \emph{concurrent} if neither precedes
the other. 
%An execution is \emph{rw-sequential} if every invocation of a read or write operation is immediately followed by a response event.
An execution is \emph{sequential} if it has no concurrent 
operations. 
An operation is \emph{complete} in $\alpha$ if the invocation event is
followed by a \emph{matching} (non-$\bot$) response or aborted; otherwise, it is \emph{incomplete} in $\alpha$.
Execution $\alpha$ is \emph{complete} if every operation is complete in $\alpha$.

For every read of object $X$ by process $p_i$ executing operation $\pi$ in $\alpha$,
we define the \emph{latest written value} of $X$ as follows:
(1) If $p_i$ contains a write to $X$ preceding the read of $X$,
then the latest written value of $X$ is the value of the latest such write to $X$.
(2) Otherwise, if $\alpha$ contains a write to $X$ by some operation $\pi'$,
$\pi'$ precedes $\pi$, and $\pi'$ is complete in $\alpha$,
then the latest written value of $X$ is the value
of the latest such write to $X$ in $\alpha$.
A sequential execution $\alpha$ is \emph{legal} 
if for every object $X$, every read of $X$ in $\alpha$ 
returns the \emph{latest written value} of $X$.
[[[\textbf{SR: Need to check this definition}]]]
An execution $\alpha$ is \emph{legal} if there exists a 

The \emph{history exported by an execution $\alpha$} is
the subsequence of $\alpha$ reduced to the invocations and responses
of operations, reads and writes, except for the reads
and writes that return $\bot$. 

\vspace{1mm}\noindent\textbf{High-level histories and linearizability.}
%\paragraph{High-level histories and linearizability.}
%
A \emph{high-level history} $\tilde H$ of an execution $\alpha$ is the subsequence of $\alpha$ consisting of all
invocations and responses of \emph{non-aborted} operations.
A complete high-level history $\tilde H$ is \emph{linearizable} with 
respect to an object type $\tau$ if there exists
a sequential high-level history $S$ equivalent to $H$ such that
(1) $\rightarrow_{\tilde H}\subseteq \rightarrow_S$ and
(2) \emph{$S$ is consistent with the sequential specification of type $\tau$}.
Now a high-level history $\tilde H$ is linearizable if it can be
\emph{completed} (by adding matching responses to a subset of
incomplete operations in $\tilde H$ and removing the rest)
to a linearizable high-level history~\cite{HW90,AW04}.

\vspace{1mm}\noindent\textbf{Obedient implementations.}
%[[ V: avoid this 
% In this paper, 
We only consider implementations that satisfy the following condition:
Let $\alpha$ be any complete sequential execution of a concurrent implementation $I$.
Then in every execution of $I$ of the form $\alpha\cdot\rho_1\cdots \rho_k$
where each $\rho_i$ ($i=1,\ldots,k$) is the complete execution of a
read, every read returns the value written by the last write that does
not belong to an aborted operation.

Intuitively, this assumption restricts our scope to
``obedient'' implementations of reads and writes, where no
read value may depend on some future write.   
In particular, we filter out implementations in which the
complete execution of a high-level operation is performed within the
first read or write of its sequential algorithm.

\vspace{1mm}\noindent\textbf{Pessimistic implementations.}
Informally, a concurrent implementation is \emph{pessimistic} if the exported history contains
every read-write event that appears in the execution. 
More precisely, no execution of a pessimistic implementation includes
operations that returned $\bot$.  

For example, a class of pessimistic implementations are those based on \emph{locks}.
A lock provides
shared or exclusive access to an object $X$ through 
synchronization primitives $\lit{lock}^S(X)$ (\emph{shared mode}),
$\lit{lock}(X)$ (\emph{exclusive mode}),  
and $\lit{unlock}(X)$.
When $\lit{lock}^S(X)$ (resp. $\lit{lock}(X)$) invoked
by a process $p_i$ returns, we say that $p_i$ \emph{holds
a lock on $X$ in shared (resp. exclusive) mode}.
A process \emph{releases} the object it holds by invoking
$\lit{unlock}(X)$.  
If no process holds a shared or exclusive
lock on $X$, then $\lit{lock}(X)$
eventually returns;
if no process holds an exclusive
lock on $X$, then $\lit{lock}^S(X)$
eventually returns; and
if no process holds a
lock on $X$ forever, then every $\lit{lock}(X)$ or $\lit{lock}^S(X)$
eventually returns. 
Given a sequential implementation of a data type, 
a corresponding lock-based concurrent one 
is derived by inserting the synchronization primitives
to provide read-write access to an object. 

\vspace{1mm}\noindent\textbf{Optimistic implementations.}
In contrast with pessimistic ones, optimistic implementations may, under
certain conditions, abort an operation:
some read or write may return $\bot$,
in which case the corresponding operation also returns $\bot$.

Popular classes of optimistic implementations are those based on
``lazy synchronization''~\cite{HHL+05,HS08-book} (with the ability of
returning $\bot$ and re-invoking an operation) or   
 \emph{transactional memory} (\emph{TM})~\cite{HM93,ST95,HLR10}.
A TM provides access to a
collection of objects via \emph{transactions}.
A transaction is a sequence of read and write operations on
objects. A transaction may \emph{commit},
or one of the read or write performed by the transaction may \emph{abort}.
Given a sequential implementation of a data type, 
a corresponding TM-based concurrent one 
puts each sequential operation within a
transaction and replaces each read and write of an object $X$ with the
transactional read and write implementations, respectively. 
If the transaction commits, then the result of the operation is
returned to the user; otherwise if one of the transactional operations aborts, $\bot$ is returned.
%

==> sequential-fix.tex <==
\begin{algorithm*}[!ht]
\caption{Sequential implementation (\textit{sorted linked list}) of \emph{set} type}
\label{alg:lists}
  \begin{algorithmic}[1]
  	\begin{multicols}{2}
  	{\size
	
	\Part{Shared variables}{
		\State Initially $\ms{head}$, $\ms{tail}$,
		\State ~~~$\ms{head}.val=-\infty$, $\ms{tail}.val=+\infty$
		\State ~~~$\ms{head}.next=\ms{tail}$
	}\EndPart
	
	\Statex
	
	\Part{$\lit{insert}(v$)}{
                \State $\ms{old} \gets \ms{head}$  		 			\Comment{copy the address}
		\State $\ms{prev} \gets \lit{read}(\ms{head})$  			\Comment{fetch the head node struct}
		\State $\ms{curr} \gets \lit{read}(\ms{prev.next})$ 		\Comment{next element is stored}
		\While{$\ms{curr.val} < v $}
                %\Comment{If the current value is less than $v$}
                       \State $\ms{old} \gets \ms{prev.next}$  \Comment{pointer to the next element}
			\State $\ms{prev} \gets \ms{curr}$ 				\Comment{move on}
%			\State $\ms{curr}\gets \ms{new}$
%			\State $\ms{curr} \gets \ms{new.next}$
			\State $\ms{curr} \gets \lit{read}(\ms{curr.next})$ 	\Comment{fetch from memory}
		\EndWhile
		\If{$\ms{curr.val} \neq v$}							\Comment{val is stored locally}
			\State $X \gets \lit{new-node}(v,\ms{prev.next})$ 	\Comment{v and addr. of curr}
%			\State $\lit{write}(\ms{prev},[\ms{old.val},X])$ 	
			\State $\lit{write}(\ms{old}, [\ms{prev.val},X])$ 	\Comment{stores val and next field}
		\EndIf
		\Return $(\ms{curr.val}\neq v)$ 						
		\EndReturn
   	}\EndPart
	
	\newpage
	
	\Part{$\lit{remove}(v$)}{

	        \State $\ms{old} \gets \ms{head}$  					
		\State $\ms{prev} \gets \lit{read}(\ms{head})$  			\Comment{fetch the head node struct}
		\State $\ms{curr} \gets \lit{read}(\ms{prev.next})$ 		\Comment{next field is stored locally}
		\While{$\ms{curr.val} < v $} 	
					\Comment{the val field is stored locally}
                       \State $\ms{old} \gets \ms{prev.next}$
                       \Comment{pointer to the next element}
			\State $\ms{prev} \gets \ms{curr}$ 				\Comment{move on}
%			\State $\ms{curr}\gets \ms{new}$
%			\State $\ms{curr} \gets \ms{new.next}$
			\State $\ms{curr} \gets \lit{read}(\ms{curr.next})$ 	\Comment{fetch from memory}
		\EndWhile
		\If{$\ms{curr.val} = v$}							\Comment{val is stored locally}
%			\State $\lit{write}(\ms{prev} ,[\ms{old.val},\ms{new.next}])$
			\State $\lit{write}(\ms{old},
                               [\ms{prev.val},\ms{curr.next}])$
%                               \Comment{next points to curr.next}
		\EndIf
		\Return $(\ms{curr.val}=v)$ 						
		\EndReturn	
   	}\EndPart
	
	\Statex
	
	\Part{$\lit{contains}(v$)}{
		\State $\ms{prev} \gets \lit{read}(\ms{head})$  			\Comment{fetch the head node struct}
		\State $\ms{curr} \gets \lit{read}(\ms{prev.next})$ 		\Comment{next field is stored locally}
		\While{$\ms{curr.val} < v $} 						\Comment{the val field is stored locally}
			\State $\ms{prev} \gets \ms{curr}$ 				\Comment{move on}
%			\State $\ms{curr}\gets \ms{new}$
%			\State $\ms{curr} \gets \ms{new.next}$
			\State $\ms{curr} \gets \lit{read}(\ms{curr.next})$ 	\Comment{fetch from memory}
		\EndWhile
 	   	\Return $(\ms{curr.val}=v)	$						\Comment{val is stored locally}
 	   	\EndReturn
   	 }\EndPart

		
	}
	\end{multicols}
  \end{algorithmic}
\end{algorithm*}

